Wireless Power Transfer with Information Asymmetry: A Public Goods Perspective

Wireless power transfer (WPT) technology enables a cost-effective and sustainable energy supply in wireless networks. However, the broadcast nature of wireless signals makes them non-excludable public goods, which leads to potential free-riders among energy receivers. In this study, we formulate the wireless power provision problem as a public goods provision problem, aiming to maximize the social welfare of a system of an energy transmitter (ET) and all the energy users (EUs), while considering their private information and self-interested behaviors. We propose a two-phase all-or-none scheme involving a low-complexity Power And Taxation (PAT) mechanism, which ensures voluntary participation, truthfulness, budget balance, and social optimality at every Nash equilibrium (NE). We propose a distributed PAT (D-PAT) algorithm to reach an NE, and prove its convergence by connecting the structure of NEs and that of the optimal solution to a related optimization problem. We further extend the analysis to a multi-channel system, which brings a further challenge due to the non-strict concavity of the agents' payoffs. We propose a Multi-Channel PAT (M-PAT) mechanism and a distributed M-PAT (D-MPAT) algorithm to address the challenge. Simulation results show that our design is most beneficial when there are more EUs with more homogeneous channel gains.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> TMC18 - arxiv/README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> TMC18 - arxiv/Sec-reference.tex <==
%!TEX root = Main-DASH-AUCTION.tex
%SourceDoc Main-DASH-AUCTION.tex

\begin{thebibliography}{99}


\bibitem{WiOpt}
M. Zhang, J. Huang, and R. Zhang, ``Wireless power provision as a public good,'' in \emph{Proc. WiOpt}, Shanghai, China, May 2018.


\bibitem{powercast}
\url{http://www.powercastco.com/}.

\bibitem{WPC}
S. Bi, C. K. Ho, and R. Zhang, ``Wireless powered communication: opportunities and challenges,'' \emph{IEEE Commun. Magazine}, vol. 53, no. 4, pp. 117-125, April 2015.

\bibitem{WPC2}
S. Bi, Y. Zeng, and R. Zhang, ``Wireless powered communication networks: an overview,'' \emph{IEEE Wireless Commun.}, vol. 23, no. 4, pp. 10-18, April 2016.

\bibitem{WPC3}
 Y. Zeng, B. Clerckx, and R. Zhang, ``Communications and Signals Design for Wireless Power Transmission," \emph{IEEE Trans. Commun.}, vol. 65, no. 5, pp. 2264-2290, May 2017.

\bibitem{6697937}
K. Huang and V. K. N. Lau, ``Enabling wireless power transfer in cellular
networks: Architecture, modeling and deployment,'' \emph{IEEE Trans. Wireless Commun.}, vol. 13, no. 2, pp. 902-912, February 2014.

\bibitem{7337464}
 S. Bi and R. Zhang, ``Placement optimization of energy and information
access points in wireless powered communication networks,'' \emph{IEEE Trans. Wireless Commun.}, vol. 15, no. 3, pp. 2351-2364, March 2016.

\bibitem{SWIPTMIMO}
R. Zhang and C. K. Ho, ``MIMO broadcasting for simultaneous wireless information and power transfer,'' \emph{IEEE Trans. Wireless Commun.}, vol. 12, no. 5, pp. 1989-2001, May, 2013.

\bibitem{6760603}
X. Zhou, R. Zhang, and C. K. Ho, ``Wireless information and power transfer in multiuser OFDM systems'',  \emph{IEEE Trans. Wireless Commun.}, vol. 13, no. 4, pp. 2282-2294, April 2014.



\bibitem{6678102}
 H. Ju and R. Zhang, ``Throughput maximization in wireless powered
communication networks,'' \emph{IEEE Trans. Wireless Commun.}, vol. 13, no. 1, pp. 418-428, January 2014.




\bibitem{6589954}
K. Huang and E. Larsson, ``Simultaneous information and power transfer for broadband wireless systems,'' \emph{IEEE Trans. Signal Process.}, vol. 61, no. 23, pp. 5972-5986, December 2013.

\bibitem{7572138}
S. Bi and R. Zhang, ``Distributed charging control in broadband wireless
power transfer networks,'' \emph{IEEE J. Sel. Areas Commun.}, vol. 34, no. 12, pp. 3380-3393, December 2016.

\bibitem{6566753}
P. Nintanavongsa, M. Y. Naderi, and K. R. Chowdhury, ``Medium access
control protocol design for sensors powered by wireless energy transfer,''
in \textit{Proc. IEEE INFOCOM}, 2013.

\bibitem{IoT}
Y. Zhang, Z. Xiong, D. Niyato, P. Wang, and D. I. Kim, ``Toward a perpetual IoT system: Wireless power management policy with threshold structure,'' \textit{IEEE Internet Things J.}, vol. 5, no. 6, pp. 5254-5270, Dec. 2018.

\bibitem{competition}
V. Gaji\'{c}, J. Huang, and B. Rimoldi, ``Competition of wireless providers for atomic users,''  \emph{IEEE/ACM Trans. Netw.}, vol. 22, no. 2, pp. 512-525, April 2014.

\bibitem{offload}
G. Iosifidis, L. Gao, J. Huang, and L. Tassiulas, ``A double-auction mechanism for mobile data-offloading markets,'' \emph{IEEE/ACM Trans. Netw.}, vol. 23, no. 5, pp. 1634-1647, October 2015.

\bibitem{Lindahl}
D. J. Roberts, ``The {Lindahl} solution for economies with public goods.'' \emph{Journal of Public Economics}, vol. 3, no. 1, pp. 23-42, 1974.

\bibitem{Micro}
A. Mas-Colell, M. D. Whinston, and J. R. Green, \emph{Microeconomic Theory}, {Oxford
  University Press}, 1995.

\bibitem{hurwicz1979outcome}
L. Hurwicz, ``Outcome functions yielding {Walrasian} and {Lindahl} allocations at {Nash} equilibrium points'', \emph{The Review of Economic Studies}, 1979.

\bibitem{sharma2012local}
S. Sharma and D. Teneketzis, ``Local public good provisioning in networks: A {Nash} implementation mechanism'', \emph{IEEE J. Sel. Areas in Commun.}, vol. 30, no. 11, December 2012.


\bibitem{chen2002family}
Y. Chen, ``A family of supermodular Nash mechanisms implementing Lindahl allocations,'' \emph{Economic Theory}, 2002.


%\bibitem{de1989stable}
%P. de Trenqualye, ``Stable implementation of {Lindahl} allocations,'' \emph{Eco-
%nomics Letters}, 1989.

\bibitem{vega1989implementation}
F. Vega-Redondo, ``Implementation of {Lindahl} equilibrium: An integration
of the static and dynamic approaches,'' \emph{Mathematical social sciences}, 1989.

\bibitem{essen2013simple}
 M. J. Essen, ``A simple supermodular mechanism that implements {Lindahl}
allocations,'' \emph{Journal of Public Economic Theory}, 2013.

\bibitem{kim1993stable}
T. Kim, ``A stable {Nash} mechanism implementing {Lindahl} allocations for
quasi-linear environments,'' \emph{Journal of Mathematical Economics}, 1993





\bibitem{saijo2010fundamental}
T. Saijo and T. Yamato, ``Fundamental impossibility theorems on voluntary participation in the provision of non-excludable public goods'', \textit{Review of Economic Design}, 2010.

\bibitem{6883469}
D. Niyato and P. Wang, ``Competitive wireless energy transfer bidding:
A game theoretic approach,'' in \emph{Proc. IEEE ICC}, 2014.

\bibitem{ref7}
P. Naghizadeh and M. Liu, ``Opting out of incentive mechanisms: A study of security as a non-excludable public good,'' \textit{IEEE Trans. Inf. Forensics Security}, vol. 11, no. 12, pp. 2790-2803, Dec. 2016.




\bibitem{powerprice}
\url{https://en.wikipedia.org/wiki/Electricity_pricing#endnote_A}


\bibitem{chiaraviglio2015life}
L. Chiaraviglio, M. Listanti, and E. Manzia, ``Life is short: The impact of power states on base station lifetime'', \textit{Energies}, 2015.

\bibitem{InterferencePrice}
J. Huang, R. A. Berry, and M. L. Honig, ``Distributed interference compensation for wireless networks,'' \emph{IEEE J. Sel. Areas Commun.}, vol. 24, no. 5, pp. 1074-1084, May 2006.

\bibitem{FCC}
\url{http://afar.net/tutorials/fcc-rules/}





%\bibitem{7264986}
%E. Boshkovska, D. W. K. Ng, N. Zlatanov, and R. Schober, ``Practical non-linear energy harvesting model and resource allocation for {SWIPT} systems'', \emph{IEEE Commun. Lett.}, vol. 19, no. 12, December 2015.

\bibitem{alphafair}
T. Lan, D. Kao, M. Chiang, and A. Sabharwal, ``An axiomatic theory of fairness
in network resource allocation,'' in \emph{Proc. IEEE INFOCOM}, 2010.




\bibitem{LTE}
\url{http://netseminar.stanford.edu/past_seminars/seminars/01_29_09.pdf.}

\bibitem{sensor} 
H. Nishimoto, Y. Kawahara and T. Asami, ``Prototype implementation of ambient RF energy harvesting wireless sensor networks,'' in \textit{Proc. IEEE SENSORS}, pp. 1282-1287, 2010.


\bibitem{WPT2}
V. Marian, B. Allard, C. Vollaire, and J. Verdier, ``Strategy for Microwave Energy Harvesting From Ambient Field or a Feeding Source,'' \textit{IEEE Trans. Power Electron.}, vol. 27, no. 11, pp. 4481-4491, Nov. 2012.
			

\bibitem{TV}
H. Nishimoto, Y. Kawahara, and T. Asami, ``Prototype implementation of ambient RF energy harvesting wireless sensor networks,'' in \textit{Proc. IEEE SENSORS}, pp. 1282-1287, 2010.



\bibitem{profit}
R. P. McAfee and P. J. Reny, ``Correlated information and mechanism design.'' \textit{Econometrica}, pp.395-421, 1993.

\bibitem{walker1980public}
M. Walker, ``On the nonexistence of a dominant strategy mechanism for making optimal public decisions.'' \emph{Econometrica}, pp.1521-1540, 1980.



%\bibitem{survey}
%J.-C. Milleron,``Theory of Value with Public Goods: A survey Article,'' \emph{Journal of Economic Theory}, 1972.
%
%\bibitem{ledyard1997public}
%J. Ledyard, ``Public goods: A survey of experimental research.'' No. 509. David K. Levine, 1997.

\bibitem{passive}
A. Mukherjee and A. L. Swindlehurst. ``Detecting passive eavesdroppers in the MIMO wiretap channel.'' in \textit{Proc. IEEE ICASSP}, 2012.



%\bibitem{DoubleAuction}
%G. Iosifidis, L. Gao, J.  Huang, and L. Tassiulas. ``A double-auction mechanism for mobile data-offloading markets,'' \textit{IEEE/ACM TON}, 2015



\bibitem{GameTheory}
R.~Gibbons,  \emph{Game Theory for Applied Economists}, {Princeton
  University Press}, 1992.



%
\bibitem{reichelstein1988game}
S. Reichelstein and S. Reiter, ``Game forms with minimal message
spaces,'' \emph{Econometrica: Journal of the Econometric Society}, 1988.

\bibitem{Meng}
M. Zhang and J. Huang, ``Efficient network sharing with asymmetric constraint information,'' \textit{IEEE J. Sel. Areas in Commun.},  vol. 37, no. 8, pp. 1898-1910, Aug. 2019.


\bibitem{CH}
C. F. Camerer, T.-H. Ho, and J.-K. Chong. ``A cognitive hierarchy model of games.'' \emph{The Quarterly Journal of Economics}, vol. 119, no. 3, pp. 861-898, 2004.

\bibitem{NUM}
D. P. Palomar and M. Chiang, ``A tutorial on decomposition methods
for network utility maximization,'' \emph{IEEE J. Sel. Areas in Commun.}, vol. 24, no. 8, pp. 1439-1451, Aug. 2006.
%








%
%\bibitem{EHsurvey}
% X. Lu, P. Wang, D. Niyato, D. I. Kim, and Z. Han, ``Wireless networks
%with RF energy harvesting: A contemporary survey,'' \emph{IEEE Communi-
%cations Surveys Tutorials}, 2015.


%\Bibitem{Saijo2010Fundamental}
%T. Saijo,  T. And Yamato,  ``Fundamental Impossibility Theorems On Voluntary Participation In The Provision Of Non-Excludable Public Goods.'' \Textit{Review Of Economic Design}, 2010.

%\bibitem{exit}
%P. Naghizadeh and M. Liu, ``Exit equilibrium: Towards understanding voluntary participation in security games,'' in \emph{Proc. IEEE INFOCOM}, 2016.




\bibitem{boyd2004convex}
 S. Boyd and L. Vandenberghe, \emph{Convex optimization}, 2004.

\bibitem{bertsekas2003convex}
D. P. Bertsekas, A. Nedi, and A. E. Ozdaglar, \emph{Convex analysis and
	optimization}, {Athena Scientific}, 2003.




%\bibitem{technical}
%Technical Report. \url{https://www.dropbox.com/s/vxo0neuinef2mig/TechnicalReport.pdf?dl=0}

\bibitem{ADAL}
N. Chatzipanagiotis, D. Dentcheva, and M. M. Zavlanos, ``An augmented Lagrangian method for distributed optimization.,'' \emph{Mathematical Programming}, vol. 152, no. 1-2, pp. 405-434, September 2015.

%\bibitem{ADAL-Conver}
%N. Chatzipanagiotis and M. M. Zavlanos, ``On the convergence rate of a Distributed Augmented Lagrangian optimization algorithm,'' in \emph{Proc. American Control Conference (ACC)}, Chicago,  pp. 541-546, 2015.
%\bibitem{Cisco}
%Cisco, ``{Cisco Visual Network Index: Global Mobile Data Traffic Forecast
%  Update},'' 2014.
%
%\bibitem{UPN2}
%R.~Sofia and P.~Mendes, ``{User-Provided Networks: Consumer as Provider},''
%  \emph{IEEE Communications Magazine}, vol. 46, no. 12, pp. 86-91, 2008.
%
%\bibitem{add-1}
%G. Iosifidis, L. Gao, J. Huang, and L. Tassiulas, ``Incentive Mechanisms for User-Provided Networks,''
% \emph{IEEE Communications Magazine}, vol. 52, no. 9, pp. 20-27, 2014.
%
%
%\bibitem{Kar}
%\url{https://yourkarma.com/}.
%
%\bibitem{opengarden}
%\url{http://opengarden.com/}.
%
%\bibitem{block}
%\url{https://en.wikipedia.org/wiki/Open_Garden}.
%
%\bibitem{au}
%\url{http://www.au.kddi.com/english/mobile/service/tethering/}.
%
%\bibitem{TetherCharge}
%S.~J. Purewal, ``{The Ultimate Android Tethering Guide}.'' [Online]. Available:
%  \url{http://www.pcworld.com/article/261928/the_ultimate_android_tethering_guide.html}
%
%
%\bibitem{fcc}
%\url{https://www.fcc.gov/document/verizon-wireless-pay-125-million-settle-investigation}.
%
%\bibitem{UKTether}
%K.~Lo, ``{Tethering on UK Networks: Which Mobile Networks Allow You To
%  Tether?}'' 2016. [Online]. Available:
%  \url{http://kenstechtips.com/index.php/tethering-on-uk-networks}
%
%\bibitem{Three}
%\url{http://www.three.co.uk/store/SIM/Plans_for_phones}.
%
%\bibitem{markendahl2013network}
%J.~Markendahl, A.~Ghanbari, and B.~G. Molleryd, ``{Network Cooperation
%  Between Mobile Operators-Why and How Competitors Cooperate?}'' \emph{Proc. IEEE IMP}, 2013.
%
%
%\bibitem{Karma}
%L.~Gao, G.~Iosifidis, J.~Huang, and L.~Tassiulas, ``{Hybrid Data Pricing for
%  Network-Assisted User-Provided Connectivity},'' \emph{Proc. IEEE INFOCOM}, 2014.
%
%\bibitem{Karma-2}
%M. M. Khalili, L. Gao, J. Huang, and B. H. Khalaj, ``Incentive Design and Market Evolution of Mobile User-Provided Networks,''
%\emph{IEEE Workshop on Smart Data Pricing}, 2015.
%
%\bibitem{Open}
%G.~Iosifidis, L.~Gao, J.~Huang, and L.~Tassiulas, ``{Enabling Crowd-Sourced
%  Mobile Internet Access},''   \emph{Proc. IEEE INFOCOM}, 2014.
%
%\bibitem{Open-2}
%G. Iosifidis, L. Gao, J. Huang, and L. Tassiulas, ``Efficient and Fair Collaborative Mobile Internet Access,"  to appear in \emph{IEEE/ACM Transactions on Networking}.
%
%\bibitem{bitcoin}
%D.~Syrivelis, G.~Iosifidis, \emph{et al.}, ``{Bits and Coins: Supporting Collaborative Consumption of
%  Mobile Internet},''   \emph{Proc. IEEE INFOCOM}, 2015.
%
%
%\bibitem{Mesh}
%R.~K. Lam, D.~M. Chiu, and J.~C.~S. Lui, ``{On the Access Pricing and Network
%  Scaling Issues of Wireless Mesh Networks},'' \emph{IEEE Transactions on   Computers}, vol. 56, no. 11, pp. 1456-1469,
%    2007.
%
%\bibitem{Mesh2}
%F.~Wu, T.~Chen, S.~Zhong, L.~E. Li, and Y.~R. Yang, ``Incentive-compatible
%  opportunistic routing for wireless networks,''  \emph{Proc. ACM MobiCom}, 2008.
%
%\bibitem{Cooper}
%L.~Chen, L.~Libman, and J.~Leneutre, ``{Conflicts and Incentives in Wireless
%  Cooperative Relaying: A Distributed Market Pricing Framework},'' \emph{IEEE Transactions on Parallel and Distributed Systems}, vol. 22, no. 5, pp. 758-772, May 2011.
%
%\bibitem{gao-1}
%L. Gao, X. Wang, Y. Xu, and Q. Zhang, ``Spectrum Trading in Cognitive Radio Networks: A Contract-Theoretic Modeling Approach," \emph{IEEE Journal on Selected Areas in Communications}, vol. 29, no. 4, pp. 843-855, April 2011.
%
%\bibitem{gao-2}
%L. Duan, L. Gao, and J. Huang, ``Cooperative Spectrum Sharing: A Contract-based Approach," \emph{IEEE Transactions on Mobile Computing}, vol. 13, no. 1, pp. 174-187, Jan. 2014.
%
%\bibitem{gao-3}
%L. Gao, L. Duan, and J. Huang, ``Two-Sided Matching Based Cooperative Spectrum Sharing," \emph{IEEE Transactions on Mobile Computing}, vol. 16, no. 2, pp. 538-551, Feb. 2017.
%
%\bibitem{energy1}
%N.~Balasubramanian, A.~Balasubramanian, and A.~Venkataramani, ``{Energy
%  Consumption in Mobile Phones: A Measurement Study and Implications for
%  Network Applications},''   \emph{Proc. ACM SIGCOMM}, 2009.
%
%\bibitem{diff}
%S.~Li and J.~Huang, ``{Price Differentiation for Communication Networks},'' in
%  \emph{IEEE/ACM Transactions on Networking}, vol. 22, no. 3, pp. 703-716, June 2014.
%
%\bibitem{tether}
%\url{http://android.stackexchange.com/questions/47819/how-can-phone-companies-detect-tethering-incl-wifi-hotspot}.
%
%\bibitem{mo2000fair}
%J.~Mo and J.~Walrand, ``Fair End-to-End Window-Based Congestion Control,''
%  \emph{IEEE/ACM Transactions on Networking}, vol. 8, no. 5, pp. 556-567, Oct 2000.
%
%\bibitem{Fair}
%T.~Lan, D.~Kao, M.~Chiang, and A.~Sabharwal, ``{An Axiomatic Theory of Fairness
%  in Network Resource Allocation},''   \emph{Proc. IEEE INFOCOM}, 2010.
%
%%\bibitem{tech}
%%{Online Technical Report}. [Online]. Available:
%%  \url{www.dropbox.com/s/8tz6uolfmz89t9i/Appendix-Tethering.pdf?dl=0}
%
%
%\bibitem{Boyd}
%S.~Boyd and L.~Vandenberghe, \emph{Convex Optimization}, Cambridge University Press, 2004.
%
%\bibitem{edgeworth}
%\url{https://en.wikipedia.org/wiki/Edgeworth_paradox}
%
%\bibitem{3Gjpb}
%L.~Wang and J.~Manner, ``{Energy Consumption Analysis of WLAN, 2G and 3G
%  Interfaces},'' \emph{Proc. IEEE/ACM GREENCOM-CPSCOM}, 2010.
%
%\bibitem{EnergyLTE}
%G.~P. Perrucci, F.~H.~P. Fitzek, and J.~Widmer, ``{Survey on Energy Consumption
%  Entities on the Smartphone Platform},''   \emph{Proc. VTC Spring}, 2011.
%
%\bibitem{4G}
%J.~Huang, F.~Qian, A.~Gerber, Z.~M. Mao, S.~Sen, and O.~Spatscheck, ``{A Close
%  Examination of Performance and Power Characteristics of 4G LTE Networks},''
%    \emph{Proc. ACM MobiSys}, 2012.
%
%\bibitem{3G}
%W.~L. Tan, F.~Lam, and W.~C. Lau, ``{An Empirical Study on 3G Network Capacity
%  and Performance},''   \emph{Proc. IEEE INFOCOM}, 2007.

\end{thebibliography}

